HDMM: Optimizing error of high-dimensional statistical queries under differential privacy

In this work we describe the High-Dimensional Matrix Mechanism (HDMM), a differentially private algorithm for answering a workload of predicate counting queries. HDMM represents query workloads using a compact implicit matrix representation and exploits this representation to efficiently optimize over (a subset of) the space of differentially private algorithms for one that is unbiased and answers the input query workload with low expected error. HDMM can be deployed for both $\epsilon$-differential privacy (with Laplace noise) and $(\epsilon, \delta)$-differential privacy (with Gaussian noise), although the core techniques are slightly different for each. We demonstrate empirically that HDMM can efficiently answer queries with lower expected error than state-of-the-art techniques, and in some cases, it nearly matches existing lower bounds for the particular class of mechanisms we consider.

==> deploy.tex <==
\newpage
\input{margexample}
\section{HDMM: Bringing it all together} \label{sec:together}

\gm{"Bringing it all together" is a little informal.  Can we rephrase the section title}

We have described the core components of HDMM - implicit representations of workloads and strategies, and efficient optimization routines that exploit these implicit representations.  In this section, we describe the remaining details of HDMM.  We give insights on how to decide which optimization operator to use, and provide efficient algorithms for the \measure and \reconstruct steps of HDMM.  We conclude with a privacy statement.   

\subsection{The $\metaopt$ strategy selection algorithm} \label{sec:sub:prog_space}

We described four optimization routines in this paper: $\optgp$, $\optk$, $\optkk$, and $\optm$.   We illustrate the behavior of each optimization operator on the simple workload of all 2-way marginals in \cref{example:margexample}.  This example highlights and summarizes the key differences between $\optk$, $\optkk$, and $\optm$.  In this case, $\optm$ is the best, which is not surprising because it is the most suitable for marginal workloads.  However, in general predicting which optimization operator will yield the lowest error strategy requires domain expertise and may be challenging for complex workloads.  Since our operators are usually efficient, we can just run each optimization operator, keeping the output strategy that offers least error.  We emphasize that strategy selection is independent of the input data and does not consume the privacy budget.  Additionally, since the strategies found by each optimization operator may depend on the initialization, we recommend running several random restarts of each optimization operator, returning the best one.

By default, we invoke all three high-dimensional optimization operators $\optk$, $\optkk$, and $\optm$.  ($\optgp$ may also be included for lower-dimensional workloads).  For $\optk$ and $\optkk$ invoked with the p-Identity strategy we use the following convention for setting the $p$ parameters: if an attribute's subworkload is completely defined in terms of $\T$ and $\I$, we set $p=1$ (this is a fairly common case where more expressive strategies do not help), otherwise we set $p=n_i/16$ for each attribute $A_i$ with size $n_i$.

\subsection{Efficient \measure and \reconstruct} \label{sec:running}

In order to run our mechanism, we need to be able to compute the matrix-vector product $ \AA \x $ for an implicitly defined strategy.  Since the strategies produced by $\optk$,$\optkk$, and $\optm$ are either Kronecker products or unions thereof, the task at hand is to efficiently compute matrix-vector products when the matrix is a Kronecker product.  

\begin{restatable}[Efficient matrix-vector multiplication]{theorem}{thmmatvec} \label{thm:matvec}
Let $ \AA = \A_1 \otimes \dots \otimes \A_d $ and let $\x$ be a data vector of compatible shape.  Then \cref{alg:fastikron} computes the matrix-vector product $\AA \x$.  Furthermore, if $\A_i \in \mathbb{R}^{n_i \times n_i}$ and $ n = \prod n_i $ is the size of $\x$ then \cref{alg:fastikron} runs in $O(n \sum n_i)$ time.  

%defined over a domain of size $ n = \prod n_i $.  Then the matrix-vector product $\AA \x$ can be evaluated in $ O(n \sum n_i)$ time.where each $\A_i$ is $n_i \times n_i$ 
\end{restatable}


\cref{alg:fastikron} is correct even if the factors of $\AA$ are not square, although the time complexity is not as clean when written down.  

\begin{algorithm}
\caption{Kronecker Matrix-Vector Product} \label{alg:fastikron}
{\small
\begin{algorithmic}[1]
\Procedure{kmatvec}{$\A_1, \dots, \A_d, \x$}
\State $m_i, n_i = $ \Call{shape}{$\A_i$}
\State $r = \prod_{i=1}^d n_i$
\State $\vect{f}_{d+1} = \x$
\For{$i = d, \dots, 1$}
\State $\matr{Z} = $ \Call{reshape}{$\vect{f}_{i+1}$, $n_i$, $r/n_i$}
\State $r = r \cdot m_i / n_i$
\State $\vect{f}_i = $ \Call{reshape}{$\A_i \matr{Z}$, $r$, $1$}
\EndFor
\State \Return $\vect{f}_1$
\EndProcedure
\end{algorithmic}}
\end{algorithm}


Since all of the strategies found by our optimization routines are either Kronecker products or unions of Kronecker products, we can efficiently implement the \measure step of HDMM using \cref{alg:fastikron}.  Computing the matrix-vector product for a union of Kronecker products is a trivial extension of \cref{alg:fastikron}: it simply requires calling \cref{alg:fastikron} for each Kronecker product and concatenating the results into a single vector.  

We can also use \cref{alg:fastikron} to efficiently implement the \reconstruct step of HDMM.  This step requires computing $\AA^+ \y$, or a pseudoinverse of $\AA$ together with a matrix-vector product.  This is done slightly differently for each type of strategy:

\begin{enumerate}
\item $\AA = \optk(\WW) = \A_1 \otimes \dots \times \A_d $.  From \cref{prop:kron} we know that $ \AA^+ = \A_1^+ \otimes \dots \otimes \A_d^+ $.  That is, the pseudoinverse of a Kronecker product is still a Kronecker product.  Thus, we can compute $\hat{\x} = \AA^+ \y$ efficiently using \cref{alg:fastikron}.  
\item $\AA = \optm(\WW) = \MM(\btheta)$.  From basic linear algebra, we know that $ \A^+ = (\A^T \A)^+ \A^T$ for any matrix $\A$.  Applied to this setting, we have $\MM^+(\btheta) = \GG^+(\btheta^2) \MM^T(\btheta)$, since we know $\MM^T \MM(\btheta) = \GG(\btheta^2)$ by \cref{prop:marggram}.  From \cref{thm:marginv} we know how to compute $\GG^+(\btheta^2)$ efficiently, and we know that it equals $\GG(\vect{\eta})$ for some $\vect{\eta}$.  We aim to compute $\MM^+(\btheta) \y = \GG^+(\btheta^2) \MM^T(\btheta) \y$.  We can easily compute $\v = \MM^T(\btheta) \y$ using a sequence of calls to \cref{alg:fastikron} by observing that $\MM^T(\btheta)$ is a just a bunch of Kronecker products \emph{horizontally} stacked together.  In a similar fashion, we can compute $\hat{\x} = \GG^+(\btheta^2) \v$ because $\GG^+(\btheta^2)$ is just the sum of a bunch of Kronecker products, which we can handle efficiently with repeated calls to \cref{alg:fastikron}. 
\item $\AA = \optkk(\WW) = c_1 \AA_1 + \dots + c_k \AA_k$.  Unfortunately, for a strategy of this form, we do not have a way to efficiently compute $\AA^+ \y$. While $\AA$ is a union of Kronecker products, the pseudoinverse is not necessarily, and we are not aware of a simple formula for the pseudoinverse of $\AA$ at all.  However, we can still produce an unbiased estimate of $\WW \x$ by using \emph{local least squares}.  To do this, we will compute $\WW_j \AA^+_j \y_j$ for each $j = 1, \dots, k$, where $\y_j$ is the answers produced for sub-strategy $\AA^+_j$.  Since $\WW_j$ and $\AA^+_j$ are both assumed to be Kronecker products, this can be easily achieved using \cref{alg:fastikron}.  This formula is an unbiased estimator for $\WW_j \x$, but the main drawback is that the workload query answers will not necessarily be consistent between sub-workloads.  
\end{enumerate}

\subsection{Improving scalability to large data vectors}

Thus far, HDMM has addressed the fundamental limitation of the matrix matrix mechanism --- replacing explicit matrix representations with implicit ones, and deriving efficient algorithms to solve the strategy optimization problem in the implicit space.  Our innovations allow HDMM to run in much higher-dimensional settings than the matrix mechanism, but HDMM still has trouble scaling to very high-dimensional settings, when the data vector no longer fits in memory.  Representing the data in vector form requires storing $ n = \prod n_i $ entries, which grows exponentially with the number of dimensions, and quickly becomes infeasible for truly high-dimensional data.  For example, a $30$-dimensional dataset with binary attributes ($n_i=2$) would require storing a data vector with $ 2^{30}$ entries, which is equivalent to approximately $ 4 \text{ GB}$ of space.   Scaling beyond this point would be quite challenging for HDMM.

It is important to note that the bottleneck of HDMM is \measure and \reconstruct, as these steps access and estimate the data vector.  In the matrix mechanism the main bottleneck is \select, as strategy optimization is the most expensive step.  HDMM can often still perform the \select step efficiently even when \measure and \reconstruct are intractable.  In some special-but-common cases, it may be possible for HDMM to bypass this bottleneck on \measure and \reconstruct, even scaling to settings where the data vector no longer fits in memory, making it suitable for arbitrarily large domains. 

The settings where HDMM can bypass this limitation depends crucially on the strategy, and consequently the workload as well.  If the workload is Identity over the whole domain (or any other full rank workload), then very little can be done because the vector of workload query answers (the output of HDMM) is just as large as the data vector itself, and simply enumerating those answers would require too much space.  Thus, the number of queries in the workload cannot be too large.  A special-but-common case occurs when the workload contains conjunctive queries over \emph{small subsets of attributes}.  The workload may cover all attributes of the dataset, but it will generally consist of a number of subworkloads, each which only cover a handful of attributes at a time.  With workloads of this form, strategies produced by HDMM ($\optkk$ and $\optm$ in particular\footnote{strategies produced by $\optk$ will generally be defined over the whole domain, rather than over a small subset of attributes}) will generally contain queries that are also defined over small subsets of attributes.  When this is the case, \measure can be done by keeping the data in its natural tabular format, and only vectorizing the data with respect to the relevant attributes for each sub-workload or sub-strategy.  Since these are assumed to be defined over small subsets of attributes, these smaller data vectors can easily be materialized explicitly and operated on accordingly.  Thus, the main remaining challenge is to \reconstruct the workload query answers while avoiding an explicit representation for $\hat{\x}$.  This can be done using a recently developed technique for efficient inference in differential privacy called ``\texttt{Private-PGM}'' \cite{mckenna2019graphical}.  \texttt{Private-PGM} consumes as input a set of noisy measurements defined over low-dimensional marginals, and produces a compact implicit representation of $\hat{\x}$.  It leverages \emph{probabilistic graphical models} to compactly represent $\hat{\x}$ in terms of a product of low-dimensional factors, and is able to scale to arbitrarily large domains as long as the measurements allow it.  

Using \texttt{Private-PGM} with HDMM does change the mechanism in some subtle but important ways.  The default HDMM method for \reconstruct is based on standard ordinary least squares, as it computes $ \hat{\x} = \AA^+ \y$, which is the solution to the minimization problem $\hat{\x}=\argmin_{\x} \norm{\AA \x - \y}_2^2$.   In contrast, \texttt{Private-PGM} is based on the related non-negative least squares problem: $\hat{\x} = \argmin_{\x > 0} \norm{\AA \x - \y}_2^2$.  We know that the true data vector is non-negative, so for this reason it seems like the \texttt{Private-PGM} approach is more natural.  However, non-negativity comes at the cost of \emph{bias}.  An appealing property of the ordinary least squares solution is that it produces an unbiased estimate of $\x$ under mild conditions.  Non-negative least squares does not share this same guarantee.  However, the introduction of bias often comes with reduced variance, and overall error is usually better when enforcing non-negativity \cite{li2015matrix,mckenna2019graphical}. 
Thus \texttt{Private-PGM} can be used not only to improve scalability of HDMM, but also utility.  In practical settings where some bias can be tolerated for reduced variance, we generally recommend incorporating \texttt{Private-PGM} post-processing into HDMM to improve utility, even when it is not necessary for scalability reasons.   

\subsection{Privacy statement}
The only step of \sys that relies on the sensitive data is \measure.  Hence, \sys inherits the privacy guarantee of the noise addition mechanism used in that step.  If  $\algG = \LM$ then \sys is $\epsilon$-differentially private by the privacy properties of the Laplace mechanism \cite{Dwork14Algorithmic}, and if $\algG = \GM$, then \sys is $(\epsilon, \delta)$-differentially private by the privacy properties of the Gaussian mechanism \cite{balle2018improving}.


==> experiments_main.tex <==
%!TEX root = paper.tex

\subsection{Accuracy comparison} \label{sec:sub:accuracy}

\newcontent{
To assess the accuracy of \sys, we considered 11 competing algorithms and a total of 12 workloads, defined over two low-dimensional datasets, two multi-dimensional datasets, and two high-dimensional datasets.  Our goal was to empirically compare error of all algorithms in all settings. However, some algorithms are not defined for some of the datasets and workloads; these cases are labeled with $\NA$ in \cref{tab:main}.  For example, a number of algorithms were designed for low-dimensions, while others were designed for high dimensions.  In addition, there are algorithms that are defined for a given dataset/workload, but were infeasible to run; these cases are labeled with $\NS$ in \cref{tab:main}. For example, in theory \matrixMech is applicable to any workload, but it is infeasible to run for the domain sizes we considered. \LRM is also applicable to any workload but is only feasible on medium-sized or smaller domains where the workload and strategy can be represented as a dense matrix. Overall, \sys and the simple baseline methods (\LMW and \Identity) are the only algorithms general and scalable enough to run in all target settings.}

\vspace{1ex}
\noindent {\bf \em Findings} \quad
\cref{tab:main} summarizes the results, reported as error ratios to \sys (so that \sys is always 1.0).  It shows that \sys is {\em never outperformed by any competing method} and offers significant improvements, often at least a factor of two and sometimes an order of magnitude.

Even when the workload is low-dimensional range queries, and we compare against a collection of algorithms designed specifically for this workload (e.g. \HB, \Privelet, \GreedyH), \sys is $1.34$ times better than the best algorithm, \HB.
% When evaluated on
On the \PermutedRange workload, only \sys offers acceptable utility,
since the other algorithms are specifically designed for (unpermuted) range queries, while \sys ad\-apts to a broader class of workloads.

Overall, we see that some algorithms approach the error offered by \sys (ratios close to 1), but, importantly, only for some experimental configurations.  To highlight this, we use bold in the table to indicate the {\em second best} error rate, after \sys.  We find that, depending on the workload and domain size, the second best error rate is achieved by a broad set of algorithms: \Identity, \HB, \Quadtree, \GreedyH are all second-best performers for some workload. This shows that some competing algorithms have specialized capabilities that allow them to perform well in some settings. In contrast, \sys outperforms across all settings, improving error and simplifying the number of algorithms that must be implemented for deployment.

In high dimensions, there are fewer competitors, and \Identity is generally the best alternative to \sys, but the magnitude of improvement by \sys can be as large as 5.79.
% for a workload consisting of a combination of low dimensional marginals and range queries.
Included in \cref{tab:main} are two data-dependent algorithms. \DAWA is defined only for 1D and 2D, but in fact timed out for some low-dimensional workloads. \PrivBayes is designed for high-dimensional data, but does not offer competitive accuracy for these datasets.  Note that the error rates for these methods may differ on different datasets (and for different $\epsilon$ values).

\eat{ %% GM: What if we deleted this stuff?
\paragraph*{Discussion} \mh{improve this discussion; point to specific results} \sys is always the most accurate algorithm, even when the workload is low dimensional range queries, and we compare against a collection of algorithms designed specifically for this task (e.g., \sys is $1.34$ times better than \HB on the \PrefixOneD workload).  The error ratio is even better on the \PrefixTwoD workload, which suggest the magnitude of improvement increasing with dimensionality, which follows theoretically from \cref{thm:err-decomp}.


}


%In additional experiments, we evaluated \sys on a larger collection of low dimensional workloads with varying domain size, and it was always the lowest-error algorithm.  We report a small representative subset of those results in the top half of \cref{tab:main}.
%
%\mh{cut?} We remind the reader that the error ratios we report for most of the algorithms we compare against hold for all datasets with the same schema, and all values of $\epsilon$.  Thus, these experimetnal comparisons are fairly comprehensive.

\subsection{Scalability comparison} \label{sec:sub:scalability}

% Commented out to compile
\begin{figure}
\centering
\subcaptionbox{\label{fig:scale1d} N/A: \DataCube}{\includegraphics[width=0.24 \textwidth]{fig/scalability-revised-1d}}
\subcaptionbox{\label{fig:scale3d} N/A: \GreedyH, \DataCube}{\includegraphics[width=0.24 \textwidth]{fig/scalability-revised-3d}}
\subcaptionbox{\label{fig:scale8d} N/A: \GreedyH}{\includegraphics[width=0.24 \textwidth]{fig/scalability-revised-8d}}
\subcaptionbox{\label{fig:scalability_run} Measure+reconstruct}{\includegraphics[width=0.24 \textwidth]{fig/scalability_mechanism.pdf}}
%\includegraphics[width=0.48 \textwidth]{fig/scalability-revised-all}
\caption{\label{fig:scalability_main}
(\subref{fig:scale1d})-(\subref{fig:scale8d}) Runtime comparison on synthetic datasets of increasing domain size (workload and dimensionality varies by plot); (\subref{fig:scalability_run}) Runtime of \sys's measure+reconstruct phase on strategies selected by its $\optk$, $\optkk$ and $\optm$ subroutines.}
\end{figure}


Next we evaluate the scalability of \sys by systematically varying the domain size and dimensionality.  We assume throughout that each dimension has a fixed size, $n$, so that $d$-dimensional data has a total domain size of $N=n^d$. We ran each algorithm on increasingly larger datasets until it exhausted memory or reached  a 30-minute timeout.

We compare against the other general-purpose algorithms: \LRM, \GreedyH, and \DataCube.  We omit \matrixMech because it cannot run at these domain sizes and \Identity, \Privelet, \HB, and \Quadtree because (as shown above) they offer sub-optimal error and specialize to narrow workload classes.
% We compare against the other general-purpose algorithms: \LRM, \GreedyH, and \DataCube.  \matrixMech is omitted because it cannot run at these domain sizes.  We also omit \Identity, \Privelet, \HB, and \Quadtree, since we have shown above that they offer sub-optimal error and specialize to narrow workload classes.

\cref{fig:scale1d} shows the scalability of \LRM, \GreedyH, and \sys on the \PrefixOneD workload.  (\DataCube is listed as not applicable (N/A) because it is not defined on non-marginal workloads.)
%
Since all three of these algorithms require as input an explicitly represented workload in dense matrix form, they are unable to scale beyond $N \approx 10^4$.  On this 1D workload, \sys runs a single instance of $\optgp$, which can be expensive as the domain size grows. \sys is more scalable than \LRM, but less scalable then \GreedyH.  (Recall \sys is run with 25 random restarts; in results not shown, we lower the number of restarts to 1.  At this setting, \sys still achieves higher accuracy than other methods yet achieves lower runtime than \GreedyH.)

\cref{fig:scale3d} shows the scalability of \LRM and \sys on the \PrefixThreeD workload. (\GreedyH is only applicable in 1D; \DataCube remains inapplicable.)  The scalability of \LRM is roughly the same in 3D as it is in 1D because it is determined primarily by the total domain size.  \sys is far more scalable in 3D however, because it solves three smaller optimization problems (for $\optk$) rather than one large problem. The main bottleneck for \sys is measure and reconstruct, not strategy optimization.

\cref{fig:scale8d} shows the scalability of \DataCube and \sys on the \ThreeWayMarginals workload (again, \GreedyH does not apply to high dimensions).  Both \DataCube and \sys ıscale well, with \DataCube scaling to domains as large as $N \approx 10^8$ and \sys scaling to $N \approx 10^9$.  On small domains, \DataCube is faster than \sys, due to \sys's higher up front optimization cost (25 random restarts and multiple optimization programs).  As the domain size grows, measure and reconstruct becomes the bottleneck for both algorithms.  A single data point is shown for \LRM because it did not finish on larger domain sizes ($N \geq 3^8$).

In summary, \sys is most scalable in the multi-dimen\-sional setting, where our implicit representations speed up strategy selection.  The main bottleneck is the measure and reconstruct steps, which we now examine more closely.

Unlike strategy selection, the cost of measure+reconstruct primarily depends on the total domain size (since the data vector must be explicitly represented).  \cref{fig:scalability_run} shows the runtime of measure+reconstruct for synthetic datasets of varying domain sizes.  Since we designed specialized algorithms for each strategy type produced by \sys (as described in \cref{sec:running}), there is one line for each strategy selection subroutine. On strategies produced by $ \optk$ and $\optm$, measure+reconstruct scales to domains as large as $N \approx 10^9$---at which point, the data vector is 4 GB in size (assuming 4 byte floats).  $\optkk$ does not scale as well ($N \approx 10^8$).  This is because computing the pseudoinverse for $ \optkk $ requires iterative methods, whereas $\optk $ and $\optm$ have closed-form expressions that we exploit.
% there is a closed form expression for the pseudo inverse of strategies produced by $\optk $ and $\optm$  that we exploit, but there is nothing we can do about , so we have to resort to iterative methods to solve the least squares problem.


==> experiments_setup.tex <==
%!TEX root = paper.tex

\subsection{Experimental setup} \label{sec:sub:exp_setup}

\vspace{1ex}
\noindent {\bf \em Implementation Details} \quad 
Our Python implementation uses the L-BFGS-B algorithm \cite{byrd1995limited}, as implemented in {\small\texttt{scipy.optimize}}, as the solver for all optimization routines. Scalability experiments were done on a 4-core Intel i7 3.6GHz processor with 16GB of RAM. The parameter $p$, controlling the size of $p$-Identity strategies for $\optgp$, is set as described in \cref{sec:sub:prog_space}. In experiments not shown, we varied $p$ and found that any choice between $\frac{n}{32}$ and $\frac{n}{8}$ results in nearly the same accuracy.  In experiments, the number of restarts ($S$ in Algorithm 2) is set to 25.  We observed that the distribution of local minima across different random restarts was fairly concentrated, suggesting that far fewer than 25 restarts may be sufficient in practice.

\vspace{1ex}
\noindent{\bf \em Competing techniques} \quad 
We compare \sys against a variety of techniques from the literature.  Some algorithms are specialized to particular settings and we indicate that below.

We consider two baseline algorithms: the Laplace Mechanism (\LMW) and \Identity.  \LMW adds noise directly to each workload query (scaled to the sensitivity)~\cite{inan2016graph,johnson2017elastic}.  \Identity adds noise to the entries of the data vector, then uses the noisy data vector to answer the workload queries. \Identity and \LMW work in both low and high dimensions, on any input workload.

We also consider the two select-measure-reconstruct methods with general search spaces: The Matrix Mechanism (\matrixMech)~\cite{li2015matrix} and the Low Rank Mechanism (\LRM)~\cite{yuan2012low}.  Both of these attempt to find a strategy that minimizes total squared error on the workload queries.

 %
% The select-measure-reconstruct paradigm is exemplified by the matrix mechanism~\cite{li2015matrix}, however, strategy selection has $\Theta(N^8)$ runtime, making it infeasible in practice.  In fact, not only is optimization difficult, simply representing the explicit input and output matrices requires significant memory resources.  However, we are able to compare against the matrix mechanism when it is invoked with a fixed and compact strategy matrix, such as the Identity strategy, which we denote \Identity.

In addition to these general-purpose algorithms, we consider a number of other algorithms designed for low-dim\-en\-sions and specialized for specific workload classes. These include \Privelet~\cite{xiao2011differential}, \HB~\cite{qardaji2013understanding}, \Quadtree~\cite{cormode2012differentially}, and \GreedyH \cite{li2014data}.  These algorithms are all designed to accurately answer range queries:
\Privelet uses a Haar wavelet as the strategy, \HB uses a hierarchical strategy with branching factor that adapts to the domain size, \GreedyH uses a weighted hierarchical strategy, and \Quadtree uses a generalization of the hierarchical strategy to two dimensions.  Of the above methods, \Privelet, \HB, and \Quadtree tend to be quite scalable but have limited search spaces.  \GreedyH solves a non-trivial optimization problem making it less scalable.
%
For workloads consisting solely of marginals, we also compare against \DataCube~\cite{ding2011differentially}.  \DataCube accepts as input a workload of marginals, and returns a strategy consisting of a different set of marginals that adapts to the input through a greedy heuristic.  %We omit direct comparison with Barak et al.~\cite{barak2007privacy} since prior work has shown it does not achieve lower error than (the better of) \LMW and \Identity.

All of the algorithms described so far, with the exception of \LMW, are members of the select-measure-reconstruct paradigm.  We also consider two state-of-the-art algorithms outside of this class: \DAWA~\cite{li2014data} and \PrivBayes~\cite{Zhang2014}.  In 1- or 2-dimensions, the \DAWA algorithm uses some of its privacy budget to detect approximately uniform regions, compresses the domain, reformulates the workload, and then uses the remainder of its privacy budget to run the \GreedyH algorithm described above. \PrivBayes is suitable for multi-dimensional datasets. \PrivBayes first privately fits a Bayes\-ian network on the data and then generates a synthetic dataset by drawing samples from the Bayes\-ian network.  The synthetic data can then be used to answer the workload.  Note that both \DAWA and \PrivBayes have error rates that depend on the input data.

\vspace{1ex}
\noindent {\bf \em Datasets} \quad
\newcontent{ 
We consider six datasets, covering low, modest, and high dimensional cases.  Most of the algorithms we consider have error rates that only depend on the schema and not the dataset instance. The different schemas we consider have a large impact on the workloads that can be defined over the data and runtime complexity of algorithms.

For 1D and 2D cases, we use representative datasets from the DPBench study~\cite{hay2016principled}, \Patent and BeijingTaxiE (which we call \Taxi).
For multi-dimensional cases, we use two datasets derived from different Census products. \Census (short for Census of Population and Housing) is the dataset used as a running example throughout the paper and is described in~\cref{sec:usecase}. \CPS is a dataset released in the March 2000 Population Survey conducted by the Census~\cite{cps}; it has five discrete attributes for income, age, marital status, race, and sex.

For high-dimensional cases, we use the \Adult and Loans dataset, which were also used in the DPBench study~\cite{hay2016principled}.  These datasets contain a combination of numeric and categorical attributes, and the former were discretized into 100 bins. 

For scalability experiments we use synthetic datasets, allowing us to systematically vary the dimensionality and attribute domain sizes.  The runtime of \sys, and the other algorithms we compare against, only depends on the domain size and dimensionality of the data, and not the contents of the data vector, so we use an all-zero data vector.
}

\vspace{1ex}
\noindent{\bf \em Workloads} \quad 
% For each dataset, we evaluate algorithms on multiple input workloads.
\newcontent{
For the \Census dataset, we use the \SFOne and \SFOnePlus workloads that were introduced in~\cref{sec:usecase} and used as a motivating use case throughout the paper.  For the other datasets, we selected workloads that we believe are representative of typical data analyst interactions.  We also synthesized a few workloads that help illustrate differences in algorithm behavior.

% 1D: Width32Range, Prefix, PermutedRange
% 2D: PrefixIdentity, Prefix 2D
% High:
% CPH: SF1, SF1+
% Adult: All Marginals, 2D Marginals (change to 2-way)
% CPS: All Range-Marginals, 2D Range-Marginals
% Synth: 1d: Prefix, 3d: Prefix 3D (PxPxP), 8d: 3-way marginals
% Synth: all range, up-to 2-way marginals

For 1-dimensional datasets, we use three workloads based on range queries: \PrefixOneD, \FixedWidthRange, and \PermutedRange.
\PrefixOneD is $P$, as described in \cref{sec:sub:logical_workloads}, and serves as a compact proxy for all range queries.
The \FixedWidthRange workload contains all range queries that sum $32$ contiguous elements of the domain (i.e., it omits small ranges).
\PermutedRange is a workload consisting of all range queries right-multiplied by a random permutation matrix to randomly shuffle the elements of the domain.  This synthesized workload serves to evaluate whether algorithms can ``recover'' the obscured range query workload.

For 2-dimensional datasets, we use workloads \PrefixTwoD and \PrefixIdentity.  The \PrefixTwoD workload is just the product workload $P \times P$.
The \PrefixIdentity workload is a union of two products: $P \times I$ and $I \times P$.

For higher dimensional datasets, we use a variety of workloads built from marginals on categorical attributes and range queries on numeric attributes.
\AllMarginals contains queries for the set of $ 2^d$ marginals (for a dataset of dimension $d$); All $\leq 3$D Marginals contains queries for every $0,1,2$ and $3$-way marginal.  All Small Marginals contains queries for every marginal whose size is less than $ 5000 $, and can include $0,1,2,\dots$-way marginals.  For each of these marginals workloads, we also consider a similar workload where we replace the Identity building block with Prefix on numeric attributes (like income and age).  We call these ``Prefix Marginals''.}

% For the higher dimensional datasets, we use workloads that we believe are representative of how an analyst would iteract with the data.  For the \Census dataset, we use the \SFOne and \SFOnePlus workloads that were introduced in~\cref{sec:usecase} have been used as a motivating use case throughout the paper.
% %
% For the \Adult dataset, we use two workloads: \AllMarginals contains queries for the set of $ 2^5$ marginals, and \TwoWayMarginals contains queries for the $ \binom{5}{2}$ 2-way marginals.
% %
% For the \CPS dataset, we use two workloads: \AllRangeMarginals is a marginals-like workload, but the Identity subworkloads are replaced by range query workloads on the numerical attributes (income and age), and \TwoWayRangeMarginals is a subset of the previous workload that only contains queries over two dimensions at a time.
\vspace{1ex}
\noindent{\bf \em Error measures} \quad 

\newcontent{To compare \sys to other algorithms in terms of accuracy, we report \emph{error ratios}, which is the square root of the ratio of the $MSE$ of the competing mechanism and HDMM, as defined in \cref{def:error}.  Recall that the MSE can be computed in closed form for data-independent mechanisms, without actually running the mechanism on real data.  Further, the error ratio holds for all values of $\epsilon$ and $\delta$.  For data-dependent mechanisms (DAWA and PrivBayes), the error ratio depends on the input data and privacy parameters and cannot be computed in closed form, so we state these and estimate the ratio using 25 random trials.}


==> main_table.tex <==
%!TEX root = paper.tex

% I + W, Wavelet, \HB, \GreedyH, \Quadtree, \LRM, \DataCube, \PrivBayes, \DAWA
%\newcommand{\resultrow}[9]{#1 & \NS & #6 & \emph{\textbf{1.0}} & #2 & #3 & #5 & #4 & #9 & #7 & #8 \\}

\begin{table}[t!]
\caption{
\label{tab:main} Error  of various algorithms on low and high dimension datasets/workloads with $\epsilon=1.0$. Algorithms labeled \NA\:are not applicable for the given configuration; algorithms labeled \NS\:are not scalable to the given configuration.}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|c||ccccc|ccccc|cc|}
\hline
\multicolumn{3}{|c||}{\textbf{Configuration}} & \multicolumn{5}{c|}{\textbf{General-Purpose Algorithms}} & \multicolumn{5}{c|}{\textbf{Low-D Range Query Algorithms}} & \multicolumn{2}{c|}{\textbf{High-D Algorithms}} \\
 \multicolumn{1}{|c}{\textbf{Dataset}}                 & \multicolumn{1}{c}{\textbf{Domain / Dimensions}}                            & \textbf{Workload}            &
$\textbf{\Identity}$ & $\textbf{\LMW}$ & \textbf{\matrixMech} & \textbf{\LRM} & \textbf{\sys} &
\textbf{\Privelet} & \textbf{\HB} & \textbf{\Quadtree} & \textbf{\GreedyH} & \textbf{\DAWA} &
\textbf{\DataCube} & \textbf{\PrivBayes} \\ \hline
%\textbf{Identity} & \textbf{LM(W)} & \textbf{Wavelet} & \textbf{\HB} & \textbf{\GreedyH} & \textbf{\Quadtree} & \textbf{\LRM} & \textbf{\DataCube} & \textbf{\matrixMech} & \textbf{\sys} & \textbf{\PrivBayes} & \textbf{\DAWA} \\\hline
\multirow{2}{*}{\textbf{\Patent}} & \multirow{2}{*}{$\mathbf{d=1, N=1024}$} & \textbf{\FixedWidthRange} & 5.66 & ? & \NS & ? & 4.53 & 11.71 & 6.72 & \NA & 5.66 & ? & \NA & \NA \\
& & \textbf{\PrefixOneD} & 22.6 & ? & \NS & ? & 6.77 & 12.16 & 9.10 & \NA & 10.13 & ? & \NA & \NA \\\cline{1-3}
%& & \textbf{\PermutedRange}& ? & ? & ? & ? & ? & ? & ? & ? & ? & ? & ? & ?\\\cline{1-3}
%
\multirow{2}{*}{\textbf{\Taxi}} & \multirow{2}{*}{$\mathbf{d=2, N=65536}$} & \textbf{\PrefixIdentity} & ? & ? & ? & ? & ? & ? & ? & ? & ? & ? & ? & ?\\
& & \textbf{\PrefixTwoD} & ? & ? & ? & ? & ? & ? & ? & ? & ? & ? & ? & ?\\\hline
%
\multirow{2}{*}{\textbf{\Census}} & \multirow{2}{*}{$\mathbf{d=5, N=2 \times 10^6}$} & \textbf{\SFOne} & 
23.20 & 70.71 & \NS & \NS & 7.30 & \NA & \NA & \NA & \NA & \NA & \NA & ?\\
& & \textbf{\SFOnePlus} & 32.50 & 141.42 & \NS & \NS & 10.23 & \NA & \NA & \NA & \NA & \NA & \NA & ?\\ \cline{1-3}
%
\multirow{2}{*}{\textbf{\CPS}} & \multirow{2}{*}{$\mathbf{d=5, N=3 \times 10^5}$} & \textbf{All Marginals} &
5.38 & 45.25 & \NS & \NS & 4.85 & \NA & \NA & \NA & \NA & \NA & ? & ?\\
& & \textbf{All Prefix-Marginals}  &
98.06 & 5352117 & \NS & \NS & 40.59 & \NA & \NA & \NA & \NA & \NA & ? & ?\\\hline
%
\multirow{2}{*}{\textbf{\Adult}} & \multirow{2}{*}{$\mathbf{d=14, N=6 \times 10^{17}}$} & \textbf{All $\leq$3D Marginals} &
5352117 & 664.68 & \NS & \NS & 225.35 & \NA & \NA & \NA & \NA & \NA & ? & ?\\
& & \textbf{All 2D Prefix-Marginals} &
475602516 & 138602 & \NS & \NS & 484.07 & \NA & \NA & \NA & \NA & \NA & ? & ?\\\cline{1-3}
%
\multirow{2}{*}{\textbf{Loans}} & \multirow{2}{*}{$\mathbf{d=12, N=8 \times 10^{15}}$} & \textbf{All Small Marginals} &
3330650 & 265.87 & \NS & \NS & 100.92 & \NA & \NA & \NA & \NA & \NA & ? & ?\\
& & \textbf{All Small Prefix-Marginals} &
15340083 & 11013 & \NS & \NS & 288.29 & \NA & \NA & \NA & \NA & \NA & ? & ?\\\hline
\end{tabular}}
\end{table}


\begin{table}[t!]
\caption{
\label{tab:main2} Error  of various algorithms on low and high dimension datasets/workloads with $\epsilon=1.0$ and $\delta=10^{-6}$. Algorithms labeled \NA\:are not applicable for the given configuration; algorithms labeled \NS\:are not scalable to the given configuration.}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|c||ccccc|ccccc|cc|}
\hline
\multicolumn{3}{|c||}{\textbf{Configuration}} & \multicolumn{5}{c|}{\textbf{General-Purpose Algorithms}} & \multicolumn{5}{c|}{\textbf{Low-D Range Query Algorithms}} & \multicolumn{2}{c|}{\textbf{High-D Algorithms}} \\
 \multicolumn{1}{|c}{\textbf{Dataset}}                 & \multicolumn{1}{c}{\textbf{Domain / Dimensions}}                            & \textbf{Workload}            &
$\textbf{\Identity}$ & $\textbf{GM}$ & \textbf{\matrixMech} & \textbf{COA} & \textbf{\sys} &
\textbf{\Privelet} & \textbf{\HB} & \textbf{\Quadtree} & \textbf{\GreedyH} & \textbf{\DAWA} &
\textbf{\DataCube} & \textbf{\PrivBayes} \\ \hline
%\textbf{Identity} & \textbf{LM(W)} & \textbf{Wavelet} & \textbf{\HB} & \textbf{\GreedyH} & \textbf{\Quadtree} & \textbf{\LRM} & \textbf{\DataCube} & \textbf{\matrixMech} & \textbf{\sys} & \textbf{\PrivBayes} & \textbf{\DAWA} \\\hline
\multirow{2}{*}{\textbf{\Patent}} & \multirow{2}{*}{$\mathbf{d=1, N=1024}$} & \textbf{\FixedWidthRange} & 23.90 & ? & \NS & 10.09 & 10.09 & 14.92 & 20.08 & \NA & 23.90 & \NA & \NA & \NA \\
& & \textbf{\PrefixOneD} & 95.64 & ? & \NS & 12.93 & 12.93 & 15.49 & 27.18 & \NA & 35.59 & \NA & \NA & \NA \\\cline{1-3}
%& & \textbf{\PermutedRange}& ? & ? & ? & ? & ? & ? & ? & ? & ? & ? & ? & ?\\\cline{1-3}
%
\multirow{2}{*}{\textbf{\Taxi}} & \multirow{2}{*}{$\mathbf{d=2, N=65536}$} & \textbf{\PrefixIdentity} & ? & ? & ? & ? & ? & ? & ? & ? & ? & ? & ? & ?\\
& & \textbf{\PrefixTwoD} & ? & ? & ? & ? & ? & ? & ? & ? & ? & ? & ? & ?\\\hline
%
\multirow{2}{*}{\textbf{\Census}} & \multirow{2}{*}{$\mathbf{d=5, N=2 \times 10^6}$} & \textbf{\SFOne} & 
69.33 & 29.87 & \NS & \NS & 9.80 & \NA & \NA & \NA & \NA & \NA & \NA & ?\\
& & \textbf{\SFOnePlus} & 97.08 & 42.25 & \NS & \NS & 10.90 & \NA & \NA & \NA & \NA & \NA & \NA & ?\\ \cline{1-3}
%
\multirow{2}{*}{\textbf{\CPS}} & \multirow{2}{*}{$\mathbf{d=5, N=3 \times 10^5}$} & \textbf{All Marginals} &
16.08 & 23.90 & \NS & \NS & 7.85 & \NA & \NA & \NA & \NA & \NA & ? & ?\\
& & \textbf{All Prefix-Marginals}  &
292.93 & 844.94 & \NS & \NS & 29.48 & \NA & \NA & \NA & \NA & \NA & ? & ?\\\hline
%
\multirow{2}{*}{\textbf{\Adult}} & \multirow{2}{*}{$\mathbf{d=14, N=6 \times 10^{17}}$} & \textbf{All $\leq$3D Marginals} &
15988375 & 91.59 & \NS & \NS & 50.32 & \NA & \NA & \NA & \NA & \NA & ? & ?\\
& & \textbf{All 2D Prefix-Marginals} &
1420766966 & 1322.58 & \NS & \NS & 126.17 & \NA & \NA & \NA & \NA & \NA & ? & ?\\\cline{1-3}
%
\multirow{2}{*}{\textbf{Loans}} & \multirow{2}{*}{$\mathbf{d=12, N=8 \times 10^{15}}$} & \textbf{All Small Marginals} &
9949649 & 57.92 & \NS & \NS & 34.91 & \NA & \NA & \NA & \NA & \NA & ? & ?\\
& & \textbf{All Small Prefix-Marginals} &
45825416 & 372.83 & \NS & \NS & 99.72 & \NA & \NA & \NA & \NA & \NA & ? & ?\\\hline
\end{tabular}}
\end{table}



==> margexample_raw.tex <==
Domain size = (2,5,50,100)

operator | error \\
---------------- \\
optm     | 62886 \\
optk     | 213270 \\
opt+     |  85070 \\
identity | 300000 \\

\begin{tabular}{c|c|c}
\multicolumn{2}{c}{Query Matrix} & Expected TSE \\\hline
$\WW$ & $\begin{bmatrix}
\T \otimes \T \otimes \I \otimes \I \\
\T \otimes \I \otimes \T \otimes \I \\
\T \otimes \I \otimes \I \otimes \T \\
\I \otimes \T \otimes \T \otimes \I \\
\I \otimes \T \otimes \I \otimes \T \\
\I \otimes \I \otimes \T \otimes \T \\
\end{bmatrix}$ & $0$ \\\hline
$\mathbb{I}$ & $\I \otimes \I \otimes \I \otimes \I $ & $0$\\\hline
$\optk(\WW)$ & $\I \otimes \I \otimes \begin{bmatrix} 0.80 \I \\ 0.20 \T \end{bmatrix} \otimes \begin{bmatrix} 0.82 \I \\ 0.18 \T \end{bmatrix}$  & $0$ \\\hline
$\optkk(\WW)$ & $
\begin{bmatrix}
0.39 (\T \otimes \T \otimes \I \otimes \I) \\
0.18 (\T \otimes \I \otimes \T \otimes \I) \\
0.14 (\T \otimes \I \otimes \I \otimes \T) \\
0.13 (\I \otimes \T \otimes \T \otimes \I) \\
0.10 (\I \otimes \T \otimes \I \otimes \T) \\
0.05 (\I \otimes \I \otimes \T \otimes \T) \\
\end{bmatrix}$ & $0$ \\\hline
$\optm(\WW)$ & $\begin{bmatrix}
0.44 (\T \otimes \T \otimes \I \otimes \I) \\
0.31 (\I \otimes \I \otimes \T \otimes \I) \\
0.25 (\I \otimes \I \otimes \I \otimes \T) \\
\end{bmatrix}$ & $0$ \\
\end{tabular}



==> parameterized.tex <==
\section{Optimizing Implicit Workloads} \label{sec:kron-param}

% commented out to compile
\begin{table*}[h]
\caption{\label{tbl:opt-summary} Summary of optimization operators: input and output types, and the complexity of objective/gradient functions.}
\resizebox{\textwidth}{!}{
\begin{tabular}{ll|c|rcl|c|l}
\multicolumn{2}{c}{\bf Definition} & 
\multicolumn{1}{c}{{\bf Output strategy}} & 
\multicolumn{3}{c}{\bf Optimization Operator} & 
\multicolumn{1}{c}{{\bf Input workload}} & 
{\bf Complexity} \\  \hline\hline
\textsection \ref{sec:sub:generalpurpose} & Problem \ref{prob:gp} & 
$p$-Identity matrix & 
$\A(\matr{\Theta})$ & $\leftarrow$ & $\optgp(\W,p)$ & 
Any explicit	 $\W\!$	& 
$N^2 p$ \\ \hline

\textsection \ref{sec:sub:opt1} & Definition \ref{def:opt1}  & 
Product, $A(\matr{\Theta})$ terms &
$\AA$ & $\leftarrow$ & $\optk(\WW, \vec{p})$ 	& 
Single product	& 
$\sum_{i=1}^d n_i^2 p_i$ \\ \hline

\textsection \ref{sec:sub:unionkron} & Problem \ref{prob:sum-kron}  & 
Product, $A(\matr{\Theta})$ terms &
$\AA$ &  $\leftarrow$ &  $\optk(w_1\WW_1 + \dots + w_k\WW_k,\vec{p})$ & 
Union of products & 
$k \sum_{i=1}^d n_i^2 p_i$ \\ \hline

\textsection \ref{sec:sub:unionkron} & Definition ~\ref{def:optp}  & 
Union of products & 
$\AA_1 + \dots + \AA_l$ & $\leftarrow$ & $\optkk(\WW_{[k_1]}, \dots, \WW_{[k_l]}, \vec{p})$	&  
Union of products &  
$k \sum_{i=1}^d n_i^2 p_i $ \\ \hline
 
\textsection \ref{sec:sub:marginals} & Problem ~\ref{prob:marginal}  & 
Weighted marginals & 
$\mathbb{M}(\vect{\theta})$ &  $\leftarrow$  & $\optm(w_1\WW_1 + \dots + w_k\WW_k)$ & 
Union of products & 
$4^d$ \\ \hline \hline
\end{tabular}}
\end{table*}

We present next a series of optimization techniques for multi-dimensional workloads, exploiting the implicit workload representations presented in Section \ref{sec:implicit}.  One of the main ideas is to decompose a strategy optimization problem on a multi-dimensional workload into a sequence of optimization problems on individual attributes.  The optimization operators $\optk$, $\optkk$, and $\optm$ are each variants described below and are summarized in \cref{tbl:opt-summary}. 

\subsection{Optimizing product workloads} \label{sec:sub:opt1}

Recall that $\WW = \W_1 \otimes \dots \otimes \W_d $, for an implicit workload that is the product of $d$ sub-workloads. If $ \W_i $ is defined with respect to a domain of size $n_i$, then $ \WW$ is defined on a total domain of size of $N = \prod_{i=1}^d n_i $.  We perform strategy optimization directly on this implicit product representation by decomposing the optimization problem into a series of explicit optimizations on the sub-workloads.
%
\begin{definition}[$\optk$] \label{def:opt1}
Given workload $\WW$ and parameter vector $\vec{p}=\langle p_1 \dots p_d \rangle$, the operator $\optk(\WW,\vec{p})$ applies $\optgp$ to each sub-workload and returns a product strategy:
\begin{align*}
\optk(\WW,\vec{p}) & = \optk(\W_1 \otimes \dots \otimes \W_d, \vec{p})   \\
& \buildrel \text{d{}ef}\over = 
			 \optgp(\W_1,p_1) \otimes \dots \otimes \optgp(\W_d,p_k) \\
			& = \A_1 \otimes \dots \otimes \A_d  =  \AA
\end{align*}
\end{definition}
%
Therefore $\optk$ merely requires solving $d$ independent instances of $\optgp$ and the resulting output strategy is the product of $d$ distinct $p_i$-Identity strategies.  This decomposition has a well-founded theoretical justification. Namely, if we restrict the solution space to a (single) product strategy, so that $\A$ has the form $\AA = \A_1 \otimes \dots \otimes \A_d$, then the error of the workload under $\AA$ decomposes into the product of the errors of its sub-workloads under corresponding sub-strategies. Thus overall error is minimized when $ Err(\W_i,\A_i) $ is minimized for each $i$ and it follows that the $\optk$ program minimizes the correct objective function.
%
\begin{restatable}[Error decomposition]{theorem}{thmerrdecomp}\label{thm:err-decomp}
Given a workload $\WW = \W_1 \otimes \dots \otimes \W_d $ and a sensitivity $1$ strategy $\AA = \A_1 \otimes \dots \otimes \A_d$, the error is proportional to: 
$$ || \WW \AA^+ ||_F^2 = \prod_{i=1}^d || \W_i \A_i^+ ||_F^2 $$
%$$ Error(\WW, \AA) = \prod_{i=1}^d Error(\W_i, \A_i) $$
\end{restatable}
%
The cost of each iteration in $\optk(\WW)$ is the sum of costs of $d$ independent optimizations of the sub-workloads $\W_i$.  Since the cost of each iteration in $\optgp$ is $O(p_i n_i^2)$, the cost for $\optk(\WW)$ is $O(\sum p_i n_i^2)$.  Note that if $\WW$ were represented explicitly, each iteration in $\optgp$ would take $O(\prod_ip_i n_i^2)$.

%\amref{Note that it would be impossible to run $\optgp$ on the explicitly-represented workload whose domain is $N = \prod n_i$.}{Rather than saying it is impossible (everything is possible with sufficient compute power) state the runtime complexity of $\optgp$ with a $p$ that can capture a strategy output by $\optk$.}  \gm{I don't follow the part about $p$, but you mean we should just state the running time as $O(p(\prod n_i)^2)$ and say its infeasible?}
%
%\begin{example} With the tools we have developed so far, a valid optimization program for the SF1 workload, $W_{sf}$, first factors the workload to get a single-product approximation and then applies $\optk$. This is expressed as $\optk(F_1(W_{sf}))$. \gm{quote results in these examples?}
%\end{example}

\subsection{Optimizing unions of product workloads} \label{sec:sub:unionkron}
%Naturally, it is quite likely that a user's input workload $\W$ will not be a Kronecker product over a set of smaller sub-workloads.  One option is to try to approximate the workload by a Kronecker product, an approach we discuss further in the next section.  Below we show a generalization of the Kronecker parameterization in which a sum of Kronecker product workloads can be optimized efficiently.  More specifically, we consider 
%The program above is defined for implicit workloads expressed as a single product.  
%Each of the $k$ rows of the above matrix consists of $d$ Kronecker products, identical to the workloads in the previous subsection.  These $k$ workloads are stacked in the matrix, which has the effect of unioning the workload queries.  We use an abbreviated notation $\WW_1 + \dots + \WW_k$

We now define three approaches for optimizing implicit workloads that are (weighted) unions of products.  Each approach restricts the strategy to a different region of the full strategy space for which optimization is tractable (see \cref{tbl:opt-summary}).  The first computes a strategy consisting of a single product; it generalizes $\optk$.  The second, $\optkk$, can generate strategies consisting of unions of products.  The third, $\optm$, generates a strategy of weighted marginals.  

\vspace{1ex}
\noindent {\bf \em Single-product output strategy} \quad 
For weighted union of product workloads, if we restrict the optimization problem to a single product strategy, then the objective function decomposes as follows:
%
\begin{theorem}
Given workload $\WW_{[k]}=w_1\WW_1 \plus \dots \plus w_k\WW_k$ and strategy matrix $\AA = \A_1 \otimes \dots \otimes \A_d$, workload error is: 
\begin{equation} \label{eq:unionkron}
|| \WW_{[k]} \AA^+ ||_F^2 = \sum_{j=1}^k w_j^2 \prod_{i=1}^d || \W^{(j)}_i \A_i^+ ||_F^2 
\end{equation}
\end{theorem} 
%
This leads to the following optimization problem:

\begin{problem}[Union of product optimization]\label{prob:sum-kron}
For a workload $\WW_{[k]}=w_1\WW_1 \plus \dots \plus w_k\WW_k$ and parameter vector $\vec{p}=\langle p_1 \dots p_d\rangle$, let: 
\begin{equation*} 
\begin{aligned}
\A_i &= \underset{\{\A_i(\matr{\Theta}_i) \:|\: \matr{\Theta}_i \in \mathbb{R}_+^{p_i \times n}\}}{\text{minimize}}
& & \sum_{j=1}^k w_j^2 \prod_{i'=1}^d || \W^{(j)}_{i'} \A_{i'}^+ ||_F^2 
\end{aligned}
\end{equation*}
and form final solution strategy as $\AA = \A_1 \otimes \dots \otimes \A_d$.
\end{problem}
%
\noindent When $k=1$, Problem \ref{prob:sum-kron} returns the same solution as \cref{def:opt1}, so we use matching notation and allow the $\optk$ operator to accept a single product or a union of products, as shown in \cref{tbl:opt-summary}.  Problem~\ref{prob:sum-kron} is a coupled optimization problem, and we use a block method that cyclically optimizes $\A_1, \dots, \A_d$ until convergence.  We begin with random initializations for all $\A_i$. We optimize one $\A_i$ at a time, fixing the other $\A_{i'} \neq \A_i$ using $\optgp$ on a carefully constructed surrogate workload $\hat{\W}_i$ (equation~\ref{eq:surrogate}) that has the property that the error of any strategy $\A_i$ on $\hat{\W}_i$ is the same as the error of $\AA$ on $\WW$.  Hence, the correct objective function is optimized. %\am{Do you run one gradient descent for each $i$ in a round robin way? Or you optimize $\A_1$, $\A_2$ and so on ...? If it is the latter, do you cycle back to $\A_1$?} \gm{I think it is the former, but Ryan can confirm.}
%To do that, we optimize one $\A_i$ at a time, fixing the others.  When we do that, every term in \cref{eq:unionkron} not involving $\A_i$ can be treated as a constant.  The constant for the $j^{th}$ term is equal to $c_j = w_j^2 \prod_{i' \neq i} || \W_{i'}^{(j)} \A_{i'} ||_F^2 $.  Optimizing the strategy for this objective function is equivalent to optimizing the strategy with respect to the workload $ \hat{\W}_i $, defined below:
{\small \begin{equation} \label{eq:surrogate}
\begin{aligned} 
\hat{\W}_i = \begin{bmatrix} c_1 \W_i^{(1)} \\ \vdots \\ c_k \W_i^{(k)} \end{bmatrix}
& &
c_j = w_j \prod_{i' \neq i} || \W_{i'}^{(j)} \A_{i'}^+ ||_F
\end{aligned}
\end{equation}}
The cost of running this optimization procedure is determined by the cost of computing $ \hat{\W}_i^T \hat{\W}_i $ and the cost of optimizing it, which takes $ O(n_i^2 (p_i+k)) $ and $ O(n_i^2 p_i \cdot \text{\sc \#iter}) $ time respectively (assuming each $(\W^T \W)_i^{(j)}$ has been precomputed). As before, this method scales to arbitrarily large domains as long as the domain size of the sub-problems allows $\optgp$ to be efficient.  

%the methods described in \cref{sec:sub:generalpurpose}. 


% Removed: drastically abbreviated version included above --GM
%\ryref{These methods consume a workload $\WW_{[k]}$ in the implicit form described in equation~\ref{eq:wsum}, however, they only depend on $ \WW_{[k]} $ through $ (\W^T \W)_i^{(j)} $, and so these  matrices are computed in the first step of the algorithm.  Alternatively, they can be passed in directly if it is convenient to do so, but we assume that they have been precomputed when reporting runtime.  For a domain of size $N = n^d$ the amount of space required to store all these matrices is $ k * d * n^2 $.  If $\WW_{[k]}$ contains product terms with many queries, this representation is more compact than $ \WW_{[k]}$, but if each product term only contains a single query, then the amount of space required to store these matrices is a factor of $n$ larger than the space required to store $\WW_{[k]}$.   For the SF1+ workload each product term requires $ 80 $ kilobytes of space, so in order for these matrices to fit comfortably in memory, $k$ must be less than $ 12,500$.}{explanation of WtW}

\vspace{1ex}
\noindent {\bf \em Union-of-products output strategy} \label{sec:sub:unionkron2} \quad 
For certain workloads, restricting to solutions consisting of a single product, as $\optk$ does, excludes good strategies.  This can happen for a workload like 
$W = (R \times T) \cup (T \times R)$,
% $\WW_{[2]} = (\R \otimes \T) \plus (\T \otimes \R)$ 
for which choosing a single product tends to force a suboptimal pairing of queries across attributes. Unfortunately, we cannot optimize directly over union-of-product strategies because computing the expected error is intractable.  Nevertheless, we can use our existing optimization methods to generate high-quality union-of-product strategies. This operator takes as input a weighted union of products, partitioned into $l$ subsets. It optimizes each individually using $\optk$ and combines the resulting output strategies to form a strategy consisting of a union of $l$ products.  Below we use $K=k_1 + \dots + k_l$ (and recall notation $\WW_{[k]}$ from \cref{sec:sub:encoding}):
%
\begin{definition}[$\optkk$] \label{def:optp} Given a workload, $ \WW_{[K]} =$ \\ $\WW_{[k_1]} + \dots + \WW_{[k_l]} $, and parameter vector $\vec{p}$, the optimization routine $\optkk$ returns the union of strategies defined below: 
%\resizebox{1.0 \textwidth}{!}{
%\begin{minipage}{\linewidth}
\begin{align*}
%\optkk(\WW_{[k_1]}, \dots, \WW_{[k_l]},\vec{p}) & 
\optkk(\WW_{[K]},\vec{p}) & 
\buildrel \text{d{}ef}\over = 
\optk(\WW_{[k_1]},\vec{p})  + \dots + \optk(\WW_{[k_l]},\vec{p}) \\
& = \AA_1 + \dots + \AA_l
\end{align*}
%\end{minipage}}
\end{definition}

%
This definition could easily be extended so that each $ \AA_i $ gets a different fraction of the privacy budget, and so that each call to $\optk$ gets a different parameter vector.

%It can also be extended to solve for the optimal privacy budget allocation between $ \AA_1 $ and $ \AA_2 $.  This can be done efficiently, but we leave this to future work.

%where $ \epsilon_i $ is the portion of the privacy budget that we use on $ \AA_i$, which is chosen so that $ \sum Error(\WW_{S_i}, \epsilon_i \AA_i) $ is minimized.  Note that this is an upper bound on the true error of the workload under the strategy, since in general all of the sub-strategies can be combined to answer the workload queries, and the extra queries cannot hurt the error~\cite{li2015matrix}. The resulting optimization problem has a simple closed form solution.

%For this optimization problem, a partition of the sub-workloads into a small set of groups to be optimized together must be supplied.  In example~\ref{example:kron-sum2}, the grouping is clear but for more complex workloads that contain a large number of sub-workloads, it is not obvious how to group them.  Thus, we propose approximating the workload by factoring it into the union of $l$ products, and using one product per group.

%\begin{example}
%Yet another optimization program would factor $\W_{sf}$ into the union of $l$ products (as in the previous example) and then apply $\optkk$: that is, compute $\optkk(F_*(W_{sf},l))$.
%\end{example}

%The above methods optimize parts of the input workload independently and then simply union the resulting strategies. This simple approach works well for all of the cases we have encountered to date. However more sophisticated methods for combining the output strategies could improve solution quality further.  In \cref{sec:sub:sumkrons2}, we describe a more advanced combination method which computes optimal weights to apply to each sub-strategy.

\subsection{Optimized marginal strategies} \label{sec:sub:marginals}

Although $\optk$ or $\optkk$ can be used to optimize workloads consisting of marginals, we now describe a third optimization operator, $\optm$, which is especially effective for marginal workloads (but is applicable to any union of product workload).  A single marginal can be specified by a subset of attributes $S \subseteq [d]$ and can be expressed as the product $\A_1 \otimes \dots \otimes \A_d $ where $\A_i = \I $ if $ i \in S $ and $ \A_i = \T $ otherwise.  
%Recall from  \cref{sec:background} that each marginal is a product whose terms consist only of $\I$ or $\T$; there are $2^d$ possible marginals.  
Since there are $2^d$ subsets of $[d]$, a set of weighted marginals can be characterized by a vector $ \vect{\theta}$ of $2^d$ non-negative weights where $\theta_1$ is the weight on the 0-way marginal (i.e., the total query) and $\theta_{2^d}$ is the weight on the $d$-way marginal (i.e., the queries defining the full contingency table). We use $\mathbb{M}(\vect{\theta})$ to denote the matrix which stacks each of these $2^d$ weighted marginals.  Each marginal has sensitivity $1$ so the total sensitivity of $\mathbb{M}(\vect{\theta})$ is $ \sum \theta_i $.  We resolve the sensitivity constraint from Problem \ref{prob:direct} by moving it into the objective function, and we resolve the other constraint by forcing $ \theta_{2^d} $ to be strictly positive.  The resulting optimization problem is given below: 
%These workloads have the form given in equation ~\ref{eq:wsum} where $k = 2^d$ and $ \W_i^{(j)} = \I $ if the $i^{th}$ bit of the binary representation of $j-1$ is $1$, and $ \W_i^{(j)} = \T $ otherwise.  We propose an alternative parameterization for these workloads that is more well suited to them.  We consider strategies of the same form, but with different weights (i.e., $ \theta_i = w_i$).   
%
%{\small
%\begin{equation} \label{eq:marginals}
%%\begin{aligned}
%%\W \! = \!\begin{bmatrix} 
%%w_1 (\T \otimes \dots \otimes \T)  \\ 
%%\ddots \\ 
%%w_{2^d} (\I \otimes \dots \otimes \I) 
%%\end{bmatrix}
%%& \! &
%\M(\vect{\theta}) \!= \! \begin{bmatrix} 
%\theta_1 (\T \otimes \dots \otimes \T)  \\ 
%\ddots \\
%\theta_{2^d} (\I \otimes \dots \otimes \I) 
%\end{bmatrix}
%%\end{aligned}
%\end{equation} }
%
%\ry{should we use $\vect{\epsilon}$ instead of $\vect{\theta}$ and use privacy budget interpretation of weights?}
%Above, each block of the matrix is one marginal (the first block is the $0$-way marginal, and the last block is the $d$-way marginal).  
\begin{problem}[Marginals optimization]\label{prob:marginal}
Given a \\ workload, $\WW_{[k]} = $ $w_1\WW_1$ $ \plus \dots \plus w_k\WW_k$, let:
\begin{equation*} 
\begin{aligned}
\vect{\theta} =  \underset{\vect{\theta} \in \mathbb{R}_+^{2^d}; \theta_{2^d} > 0}{\text{minimize}}
& & \Big( \sum \theta_i \Big)^2 || \WW_{[k]} \mathbb{M}(\vect{\theta})^+ ||_F^2
\end{aligned}
\end{equation*}
\end{problem}
%
Without materializing $\mathbb{M}(\vect{\theta})$ we can evaluate the objective function and its gradient by exploiting the structure of $\mathbb{M}(\vect{\theta})$.  For strategies of the form $\mathbb{M}(\vect{\theta})$, $ (\mathbb{M}^T \mathbb{M})^+ $ can be written as the weighted sum of $ 2^d $ kronecker products, where each sub-matrix is either $ \I $ or $\matr{1} = \T^T \T $, and we can efficiently find the $2^d$ weights that characterize the inverse by solving a (sparse) linear system of equations.  The objective function only depends on $\WW_{[k]}$ through the trace and sum of $ (\W^T \W)^{(j)}_i $.  Thus, these statistics can be precomputed for the workload and the objective function can be evaluated very efficiently. The cost of this precomputation is linear in $k$, but subsequent to that, evaluating the objective and gradient only depends on $d$, and not $n_i$ or $k$.  Specifically, the time complexity of evaluating the objective and gradient is $O(4^d)$ -- quadratic in $2^d$, the size of $\vect{\theta}$.  %Experiments show that this parameterization is scalable up to 16 dimensions.

%and the weights $w_i$ can be 0 to exclude a marginal, 1 to include a marginal, or, more generally, can specify the relative importance of the included marginals.  Since a highly weighted marginal contributes more to the aggregate error, the optimization problem will favor solutions in which the error on that marginal is comparatively lower.  Accordingly, for the strategy $\A(\theta)$, the weight $\theta_i$ will determine the (relative) scale of the noise added to the $i^{th}$ measured marginal.  

%We can efficiently solve the optimization problem for this workload under this parameterization.  In fact, as we will show, we can evaluate the objective function in quadratic time with respect to $2^d$, which is a huge improvement over the direct methods which require cubic time with respect to $n$.  For non-binary domains, $n$ is much larger than $2^d$. 

%\begin{table}[H]
%\begin{operator}[$\optm$] \hfill \\
%\begin{outline}
%\0 Usage: $\MM^d_1 + \dots + \MM^d_k \leftarrow \optm(w_1\WW_1 + \dots + w_k\WW_k)$ \\
%\0 Input: union of products\\
%\0 Output: weighted marginals\\ 
%\end{outline}			
%\end{operator}
%\end{table}
%
%\todo{state complexity}
%
%\begin{example}
%The final optimization program could approximate $\W_{sf}$ by a union of products and apply $\optm$: that is, compute $\optm(F_*(W_{sf}, k))$.
%\end{example}
%

%The general purpose parameterization described in the last section scales to domains as large as 8192.  In this section, we introduce the Kronecker parameterization, which is designed for much larger multi-dimensional domains.  

%\begin{align}
%\A & \leftarrow \optgp(\W,p) \tag{a}\\
%\AA & \leftarrow \optk(\WW, \vec{p}) \tag{b} \\
%\AA & \leftarrow \optk(\WW_1 + \dots + \WW_k) \tag{c} \\
%\AA_1 + \dots + \AA_k & \leftarrow \optkk(\WW_1 + \dots + \WW_k) \tag{d}
%\end{align}




%\begin{table}[H]
%\begin{operator}[$\optk$] \hfill \\
%\begin{outline}
%\0 Usage: $\AA \leftarrow \optk(\WW)$ \\
%\0 Input: $\WW$ Kronecker product workload, implicit \\ 
%\0 Output: $\AA$, Kronecker strategy, implicit\\ 
%\end{outline}			
%\end{operator}
%\end{table}

%Suppose $\W$ is a workload that is the Kronecker product of $d$ sub-workloads: $\W = \W_1 \otimes \dots \otimes \W_d $.  If we restrict the solution space to strategies that are also Kronecker products, so that $\A = \A_1 \otimes \dots \otimes \A_d$, we find that the objective function decomposes nicely. 

%\begin{example}
%	As a simple example of the application of this theorem, recall the census workload described earlier.  The Summary File 1 queries are defined in terms of 5 attributes (sex, age, hisp, race, relation) and consist of 4151 queries.  When evaluated in this form, they represent national-level statistics about demographic characteristics.  Call this workload $\W_{sf}$.  If we wish to release the 4151 for {\em each} state, then the workload consists of $50 \times 4151$ queries represented by $\I \otimes \W_{sf}$, where $\I$ is the Identity on the State attribute.  Since $\I$ is the optimal strategy for the workload $\I$, Theorem \ref{thm:err-decomp} suggests that we can consider strategies of the form $\I \otimes \A_{sf}$ where $\A_{sf}$ is an optimized strategy for $\W_{sf}$.  Even this simple application of the theorem means we can optimize a workload over a domain of $500,000$ instead of $25,000,000$.  (Further analysis of the optimization of $\W_{sf}$ is included in the running examples below.)
%	\gm{this ex. needs to be polished and synced with rest of examples.}
%\end{example}

%\gm{say explicitly somewhere that $\W_i$ and $\A_i$ do not nec. need to be over one dimension? could combine dimensions}

%\ry{somewhere here: this error decomposition is strong justification for considering kronecker product strategies}

%\subsection{Kronecker parameterization} \label{sec:sub:single-kron}
%
%The error decomposition is strong justification for considering Kronecker product strategies.  We therefore combine that insight with the techniques from section~\ref{sec:optimization} and optimize over strategies of the form:
%%
%\begin{equation} \label{eq:kronparam}
%\A(\matr{\Theta}) = \A(\matr{\Theta}_1) \otimes \dots \otimes \A(\matr{\Theta}_d)
%\end{equation}
%%
%where each $\A(\matr{\Theta}_i)$ is a $p$-Identity strategy defined by parameters $\matr{\Theta}_i$.  Thus the overall optimization problem, described below, consists of solving $d$ instances of Problem \ref{prob:gp}:
%
%\begin{problem}[Single Kronecker optimization]\label{prob:single-kron}
%Given a workload matrix $\W = \W_1 \otimes \dots \otimes \W_d $ and hyper-parameter vector $\vec{p}=\langle p_1 \dots p_d\rangle$, let:
%\begin{equation*} 
%\begin{aligned}
%\A_i &= \underset{\{\A(\Theta) \:|\: \Theta \in \mathbb{R}_+^{p_i \times n}\}}{\text{minimize}}
%& & || \W_i \A_i^+ ||_F^2 \\
%\end{aligned}
%\end{equation*}
%and form final solution strategy as $\A = \A_1 \otimes \dots \otimes \A_d$.
%\end{problem}

%\begin{example}
%	\gm{Or an example of a large multi-dimensional domain and some concrete runtime numbers for how quickly we can optimize using this decomposition.  Forward pointer to some numbers from experiments.}
%\end{example}

%\begin{table}[h]
%\begin{operator}[$\optk$] \hfill \\
%\begin{outline}
%\0 Usage: $\AA \leftarrow \optk(w_1\WW_1 + \dots + w_k\WW_k,\vec{p})$ \\
%\0 Input: Union of products\\
%\0 Output: (Single) product of $p$-Identity matrices\\ 
%\end{outline}			
%\end{operator}
%\end{table}

%\begin{remark}
%The time complexity of evaluating the objective and gradient only depends on the domain size of each dimension, and not the overall domain size.  Thus, the optimization problem can be solved for arbitrarily large domains by scaling out the number of dimensions.
%\end{remark}

%In the special case when $k=1$, this procedure can be simplified to optimizing $\A_i$ for the workload $\W^{(1)}_i $ for each $i$ since the optimization problem for a workload $\W$ is equivalent to the optimization problem for a workload $c\W$ up to a constant factor.

%\begin{example}
%An alternative optimization program factors using $F_*(\W_{sf},k)$ and then uses $\optk$ on the resulting union of $k$ products.  $\W_{sf}$ can be factored with zero deviation when $k=32$, or can be approximated with smaller $k$, trading off efficiency for precision of the objective function.
%\end{example}


%
% We provide an intuitive example below.
%\begin{example} \label{example:kron-sum2}
%Consider the following 2D workload, $\W$, which contains all 1D range queries (on each dimension of an $n \times n$ domain).  \todo{give better intuitive explanation of this workload for reader}
%%
%$$ \W = \begin{bmatrix} \R \otimes \T \\ \T \otimes \R \end{bmatrix}  \qquad
%\A = \begin{bmatrix} \B \otimes \T \\ \T \otimes \B \end{bmatrix}
%$$ 
%The optimal strategy should be near $\A$ above, where $\B$ is the strategy that optimizes $\R$.
%%It will probably be slightly different because some information is shared between the $B \otimes T$ queries and the $T \otimes B$ queries.  In particular, a noisy estimate of the query $T \otimes T$ can be obtained from both parts of the strategy, and this extra information can influence what the queries in $B$ should be.	
%However, it would be impossible to find $\A$ using $\optk$ since it is not a single product.  A close single-product approximation of $\A$ would have the following form:
%$$ \begin{bmatrix} \B \otimes \B \\ \B \otimes \T \\ \T \otimes \B \\ \T \otimes \T \end{bmatrix} = \begin{bmatrix} \B \\ \T \end{bmatrix} \otimes \begin{bmatrix} \B \\ \T \end{bmatrix} $$
%and $\optk$ would be able to find something similar. However, the extra queries in $\B \otimes \B$ (and $\T \otimes \T$) raise the sensitivity of the strategy without improving error on the workload queries much, which leads to unnecessarily high error.  
%\end{example}
%

%\ry{it would be nice if we could describe $\optkk$ as consuming $l$ parameter vectors, but do we have space?}   NOPE! --GM

%
%{\small
%\begin{tabular}{llccc}
%\multicolumn{3}{l}{$\optkk(\WW_{[k]}) = \optk(\WW_{[j]}) + \optk(\WW_{[j+1,k]})$} & \\
%\multicolumn{3}{l}{$\optkk(w_1\WW_1 + \dots + w_j\WW_j + w_{j+1}\WW_{j+1} + \dots + w_k\WW_k) $} & \\
%$\buildrel \text{d{}ef}\over = $ & $\optkk(w_1\WW_1 + \dots + w_j\WW_j) \,\, + $  & \\
%  & $\optkk(w_{j+1}\WW_{j+1} + \dots + w_k\WW_k)$ & $=\,\,\AA_1 + \AA_2$ & 
%\end{tabular} }

%\begin{align*}
% \optkk(w_1\WW_1 + \dots + w_k\WW_k) & 
% \buildrel \text{d{}ef}\over = 
% \epsilon_1 \optk(\WW_{S_1}, \vec{p}_1) + \dots + \epsilon_l \optk(\WW_{S_l}, \vec{p}_l) \\
% 		& = \epsilon_1\AA_1 + \dots + \epsilon_l\AA_l 
%\end{align*}	
%


==> query_formalism.tex <==
\section{Query Formalism}

\ry{this is a temporary section to keep latex files clean}

Let the database $D$ be an instance of a single-relation schema $ R(\mathbb{A}) $ with attributes $\mathbb{A} = \set{\mathcal{A}_1, \dots, \mathcal{A}_d} $.  
\ry{need to reformulate this to make sure definitions 4-6 make sense}

\begin{definition}[Data Vector]
For an ordered list of disjoint cell conditions $ \phi_1^{\mathbb{A}}, \dots, \phi_n^{\mathbb{A}} $, the data vector $x$ is a $n \times 1 $ column vector where $ x_i = | \set{t \in D \mid \phi_i^{\mathbb{A}}(t)} | $.  
\end{definition}

Informally, $ x_i $  counts the number of the tuples in the database satisfying condition $ \phi_i $. 
\begin{definition}[Linear Query]
A linear query is a $ 1 \times n $ row vector $ q $ where the answer to the linear query is the dot product $ q x = q_1 x_1 + \dots + q_n x_n $.  
\end{definition}

If $q$ is a binary vector, then it represents a predicate counting query - it counts how many tuples in the database satisfy any of the cell conditions specified by $q$. 

\begin{definition}[Query Matrix]
A query matrix is a collection of linear queries $ q_1, \dots q_m $ organized into the rows of a $ m \times n $ matrix.  
\end{definition}

For multi-dimensional data, the cell condition $ \phi_i $ is usually a conjunction of cell conditions on each attribute.  With this in mind, it is sometimes convenient to organize the data into a matrix instead of a vector.  This enables us to reason about a special class of query matrices which will become important later. 

\ry{explain why we need two sets of attributes}
\begin{definition}[Data Matrix]
For cell conditions $ \phi_i^{\mathbb{A}} $ and $ \phi_j^{\mathbb{B}} $ defined over disjoint sets of attributes $ \mathbb{A} $ and $ \mathbb{B} $ respectively, the data matrix $X$ is a matrix where $ X_{ij} = | \set{t \in D \mid \phi_i^{\mathbb{A}}(t), \phi_j^{\mathbb{B}}(t)} | $.  The corresponding data vector is $ x = vec(X) $, where $vec$ flattens a matrix into a column vector in row-major order, and the element of $x_k$ corresponding to $X_{ij}$ has cell condition $ \phi_k^{\mathbb{A} \mathbb{B}} = \phi_i^{\mathbb{A}} \wedge \phi_j^{\mathbb{B}} $.
\end{definition}

This data matrix is nothing more than an intermediate representation that is useful to the discussion that follows.  It's easy to go back and forth between the two representations by flattening and reshaping the data.  We will sometimes refer to the $ mat $ as the inverse operation of $vec$, which turns a data vector into a data matrix where the shape is implied by the context.  It's also possible to generalize the data matrix and organize $d$-dimensional data as a rank-$d$ tensor, although doing so is not necessary for the discussion that follows.

\begin{definition}[Query Intersection]
For queries $a$ and $b$ defined over disjoint sets of attributes $\mathbb{A}$ and $\mathbb{B}$, a data matrix $X$ and an associated data vector $vec(X)$, the query intersection $a \sim b$ maps two linear queries defined over $ \mathbb{A} $ and $ \mathbb{B} $ into a linear query defined over $ \mathbb{A} \cup \mathbb{B} $ such that
$$ (a \sim b) vec(X) = \sum_{i,j} a_i b_j X_{ij} $$
which can be computed compactly as $ a X b^T $.   
\end{definition}

If $a$ and $b$ both represent predicate counting queries, then $ a \sim b $ also represents a predicate counting query that counts how many tuples in the database satisfy the predicates from both $a$ and $b$.  Of course, this notion of query intersection generalizes to all linear counting queries, not just predicate counting queries. Nevertheless, it gives us a nice way to think about the operation.  

\begin{definition}[Cartesian Product in Query Space]
For query matrices $A$ and $B$ defined over disjoint sets of attributes $\mathbb{A}$ and $\mathbb{B}$, the cartesian product in query space, denoted $ A \otimes B $ contains the query intersection of every pair of queries from $A$ and $B$
\end{definition}

According to proposition~\ref{prop:kron} $ A \otimes B $ using Kronecker products.  

\begin{proposition} \label{prop:kron}
The cartesian product in query space between $A$ and $B$ can be obtained by computing the Kronecker product between $A$ and $B$.  
\end{proposition}

\begin{proof}
Let $X$ be the data matrix and $ vec(X) $ be the associated data vector.  Note that $ A X B^T $ represents the answers to the desired set of queries, since $ (A X B^T)_{ij} = a_i X b_j^T $, which is the query intersection between $a_i$ and $b_j$.  The matrix equations identity for kronecker products states that $ (A \otimes B) vec(X) = vec(A X B^T) $, so $ A \otimes B$ represents the desired set of queries for the data vector $ vec(X) $, where $ \otimes $ is the Kronecker product.  
\end{proof}

It's easy to extend the results to show that query matrices can be constructed from the kronecker product of more than two matrices.  This is done by inductively applying proposition~\ref{prop:kron} with new query matrices.  For example, we could apply the proposition to show that the cartesian product in query space between $(A \otimes B) $ and $ C $ is $ (A \otimes B) \otimes C $.  Since $ \otimes $ is associative, the order that we arrange the parentheses doesn't matter and we can just write the query matrix as $ A \otimes B \otimes C $.   A common case is to have one sub query matrix per attribute so that $ A_i $ is the query matrix for the set of attributes $ \set{\mathcal{A}_i} $.   

These definitions give us a natural and compact way to represent many important high-dimensional workloads. 
 

